LiTe-GS: Oracle-Efficient Next Best View Selection for 3D Gaussian Splatting

Selecting informative camera views is critical for efficient training and adaptive refinement in 3D Gaussian Splatting, where each observation significantly influences model parameters. However, information-driven view-selection strategies can require repeated evaluations of expensive information-gain oracles as the number of candidate views increases. We propose LiTe-GS, an oracle-efficient method for next best view selection in 3D Gaussian Splatting. LiTe-GS reduces the number of information-oracle evaluations by performing randomized subset evaluation of candidate views rather than exhaustively scoring the full candidate pool. The resulting approach achieves expected $O(M\log(1/\epsilon))$ oracle complexity with respect to the number of candidate views $M$, independent of the selection cardinality $K$, while providing an explicit trade-off between oracle efficiency and approximation quality through $\epsilon$. We provide theoretical guarantees on oracle complexity and approximation performance under the proposed selection scheme. Experiments on Blender and Mip-NeRF 360 demonstrate that LiTe-GS maintains reconstruction quality comparable to Fisher-information-based baselines while substantially reducing the number of Fisher-oracle evaluations across different acquisition settings.

==> sec/8_rebuttal.tex <==

\section{Rebuttal}
\noindent\textbf{Algorithmic novelty.}
We do not claim stochastic greedy or lazy evaluation as new generic optimization techniques. LiTe-GS specializes these established mechanisms to Fisher-information-based NBV selection in 3DGS, where marginal-gain evaluation requires an expensive block-diagonal Fisher oracle. Randomized candidate-subset evaluation yields expected $O(M\log(1/\varepsilon))$ oracle complexity, independent of $K$, versus $O(MK)$ for exhaustive greedy selection, with the corresponding approximation guarantee. Moreover, $\varepsilon$ provides a user-controlled trade-off between approximation quality and oracle expenditure. Thus, our contribution is the resulting problem-specific oracle-efficient NBV formulation and its complexity/approximation characterization, rather than novelty in stochastic or lazy greedy optimization.

\vspace{0.21cm}

\noindent\textbf{FisherRF comparison.}
FisherRF uses a diagonal Fisher approximation, with $O(Nd)$ retained entries, whereas POP-GS/LiTe-GS use a $d\times d$ block per Gaussian, with $O(Nd^2)$ entries. Their oracle evaluations therefore correspond to different computational objects and are not directly comparable as per-evaluation costs. The selection mechanism itself is representation-agnostic: reducing the block-diagonal approximation to its diagonal reduces POP-GS to the FisherRF-style oracle, and LiTe-GS correspondingly becomes randomized-subset selection over that oracle. Our claim is therefore reduction in Fisher-oracle evaluations, irrespective of the underlying Fisher representation.

\vspace{0.21cm}

\noindent\textbf{Oracle accounting and ablation scope.}
LiTe-GS does not perform an initial exhaustive $O(M)$ Fisher evaluation: each acquisition stage first samples a subset and evaluates only that subset. We corrected the marginal-gain initialization in the algorithm accordingly. Reported counts are conservative worst-case counts, charging every sampled candidate as an evaluation; lazy evaluation can only reduce the realized count. The SSG ablation isolates dynamic randomized resampling: LiTe-GS resamples at each stage whereas SSG keeps the subset fixed, with all other conditions identical. We additionally evaluate this ablation on Mip-NeRF~360/Garden alongside Blender/Ship.

\vspace{0.21cm}

\noindent\textbf{Oracle efficiency and scalability.}
Our efficiency claim is scoped to the information-driven NBV selection module (Box~3 in Fig.~2), where Fisher-information evaluation is the oracle. Random selection bypasses this module and hence incurs no Fisher-oracle evaluations. We claim \emph{oracle}, not wall-clock or end-to-end, efficiency: oracle complexity is implementation- and hardware-independent and directly measures information evaluations requested by the selector. Scalability refers to controlling this expenditure through $\varepsilon$ as the candidate pool grows, rather than to universal end-to-end runtime improvement.

\vspace{0.21cm}

\noindent\textbf{Datasets and experimental settings.}
The experiments test whether oracle-efficiency reduction persists across scenes, datasets, and acquisition protocols rather than provide an exhaustive benchmark sweep. We evaluate three Blender and three Mip-NeRF~360 scenes under two acquisition setups, yielding numerous paired POP-GS--LiTe-GS comparisons with consistent oracle reduction. The 3DGS/Fisher configurations are representative, not claimed optimal; LiTe-GS and POP-GS use identical candidate pools, initialization, acquisition protocol, training schedule, and parameter settings. Thus, changing common settings may alter absolute reconstruction quality but does not confound the relative comparison. The view-selection framework is built on the FisherRF repository.

\vspace{0.21cm}

\noindent\textbf{Changes in the revision.}
In response to the reviewers, we (i) add an ablation over different
selection cardinalities $K$, (ii) extend the dynamic-resampling versus
SSG ablation from Blender/Ship to Mip-NeRF~360/Garden, (iii) expand the
$\varepsilon$ sensitivity study, (iv) correct and clarify the oracle
initialization and conservative oracle accounting, and (v) clarify the
FisherRF comparison, experimental scope, and contribution statements.
Additional implementation details and experimental results are provided
in the supplementary material.
